ARM-Net: Adaptive Relation Modeling Network for Structured Data

Relational databases are the de facto standard for storing and querying structured data, and extracting insights from structured data requires advanced analytics. Deep neural networks (DNNs) have achieved super-human prediction performance in particular data types, e.g., images. However, existing DNNs may not produce meaningful results when applied to structured data. The reason is that there are correlations and dependencies across combinations of attribute values in a table, and these do not follow simple additive patterns that can be easily mimicked by a DNN. The number of possible such cross features is combinatorial, making them computationally prohibitive to model. Furthermore, the deployment of learning models in real-world applications has also highlighted the need for interpretability, especially for high-stakes applications, which remains another issue of concern to DNNs. In this paper, we present ARM-Net, an adaptive relation modeling network tailored for structured data, and a lightweight framework ARMOR based on ARM-Net for relational data analytics. The key idea is to model feature interactions with cross features selectively and dynamically, by first transforming the input features into exponential space, and then determining the interaction order and interaction weights adaptively for each cross feature. We propose a novel sparse attention mechanism to dynamically generate the interaction weights given the input tuple, so that we can explicitly model cross features of arbitrary orders with noisy features filtered selectively. Then during model inference, ARM-Net can specify the cross features being used for each prediction for higher accuracy and better interpretability. Our extensive experiments on real-world datasets demonstrate that ARM-Net consistently outperforms existing models and provides more interpretable predictions for data-driven decision making.

==> secs/0.response.tex <==
\newcommand{\comments}[2]{\noindent\underline{\textbf{Comment #1}}: \emph{#2}}
\newcommand{\response}[1]{\vspace{1mm}\noindent\textbf{RESPONSE}: #1\vspace{1mm}}
\newcommand{\responseArg}[2]{\vspace{1mm}\noindent\textbf{RESPONSE #1}: #2\vspace{1mm}}
\newcommand{\revhighlight}[1]{\emph{\textbf{\uuline{#1}}}}
\pagestyle{empty}
\thispagestyle{empty}

% \newcommand{\question}[1]{}
\newcommand{\question}[1]{{\textcolor{blue}{(#1)}}}

\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{10mm}

\begin{multicols}{2}

\setcounter{page}{1}

\noindent Dear Reviewers,

\vspace{5mm}
We would like to thank the meta reviewer and reviewers for your constructive comments, which have indeed helped to raise the quality of this paper.
In this cover letter, we will first summarize the major changes that we have made in the revised manuscript, and then respond to each concern raised by reviewers.
\rev{We highlight major changes in blue in the manuscript.}

\section*{Summary of Changes}
\begin{itemize}[leftmargin=*]
	
	\item We have toned down the interpretability of \name by updating the discussion around explainability in Abstract and Introduction and moving the detailed discussion to a separate subsection in Section~\ref{sec:analysis_and_discussion}.

    \item We have clarified our design choices and rationales behind each module of \name in highlighted paragraphs of Introduction, Section~\ref{sec:overview}, Section~\ref{sec:architecture} and Section~\ref{sec:analysis_and_discussion}.

    \item We have introduced an example in Introduction (highlighted in blue in the sixth paragraph of Section 1) to improve the clarity.
    
    \item We have related our approach in term of XAI taxonomies in the newly introduced \textit{Interpretability} subsection in Section~\ref{sec:analysis_and_discussion}, and compared the interpretability results of \name against two general interpretation approaches (Lime~\cite{lime} and Shap~\cite{shap}) in Section~\ref{sec:exp_interpretability}.
    
    \item We have introduced DNN and two GNN models (GCN~\cite{gcn} and GAT~\cite{gat}) as new baselines in Section~\ref{sec:baseline}, included their results in the overall prediction performance summarized in Table~\ref{tab:overall_resutls} and updated the effectiveness discussions in Section~\ref{sec:exp_effectiveness} accordingly.
    
    \item We have updated the implementation of all the baseline models and evaluated the effectiveness of all the models with the same updated training settings, which is introduced in Section~\ref{sec:hyper_settings}.

    \item We have updated the entire interpretability section of Section~\ref{sec:exp_interpretability} and rearranged the interpretation results into three subsections, namely \textit{Interpretability Settings}, \textit{Global Interpretability} and \textit{Local Interpretability}.
    
    \item We have greatly reduced the experimental evaluation on interpretability in Section~\ref{sec:exp_interpretability} to make space for additional experiments, namely \textit{NN-based Models and Ensemble Models}, \textit{Efficiency}, \textit{Enhancing FM with Exponential Neurons}, \textit{Multi-Head Attention and Sparsity} and \textit{Enhancing \nameplus with a Larger Embedding Size} in Section~\ref{sec:exp_effectiveness} and Section~\ref{sec:exp_ablation}.

\end{itemize}

\section*{Response to Meta-Reviewer}
\comments{Meta-Reviews}{
%The consensus is to allow the authors to submit a revised version in order to address the points raised in the reviews.
The reviews point out what is needed in the revision (see field 13 in the reviews).
In addition, there was some discussion about how the numbers of the baseline are copied from other papers and hence it's unclear whether they provide an apples-to-apples comparison with the experiments reported in the paper. To ensure comparability, the revision should instead run evaluate the baselines using the same experiments as the proposed method.
}

\response{
We have revised our manuscript accordingly to address the concerns raised by all the reviewers.

For the baselines, we adopted the same benchmark datasets (except \diabetes) and training settings as AFN~\cite{afn}, which are indicated in Sec 4.1.5 Implementation Details of the original manuscript (\textit{tune all other hyperparameters on the validation set following AFN}).
As a consequence, many results are consistent with the AFN paper in the original manuscript.
% Since our experimental results are consistent with the AFN paper, we thus decided to report the numbers in the AFN paper for the four datasets for consistency.
%%% ooibc: this is a funny thing to do
%%%% just report ours, and say explicitly that they are consistent with the AFN paper's.
%%% else sound fishy

In the revised manuscript, we have updated the implementation of all the baseline models and adopted three neural network based baselines as suggested by the reviewers.
Further, for a fair comparison, we evaluate the effectiveness of all the models with the same updated training settings, which is introduced in Section~\ref{sec:hyper_settings}.
The updated results reported in this manuscript are obtained by a thorough grid search of hyperparameters for all the models (over 10k runs in total), each with five independent runs to reduce randomness.
We will provide all the implementation and datasets for reproducibility.
}

\section*{Response to Reviewer 1}
\comments{O1}{The paper should better justify the design decisions of ARM-Net. First, would not a layer which learns relational embeddings instead of using hard-coded embeddings be an interesting alternative and be a more general solution?}

\response{We note that all the embedding weights are learnable parameters, and thus the preprocessing module actually learns relational embeddings.}
% comments updated by this reviewer: the author feedback clarified individual comments of my original review (e.g. O1)

\comments{O2}{I also had a similar question why graph neural networks for relational databases (e.g., [15]) would not learn cross-features efficiently since they also adjust weights on a per-tuple basis and in addition to ARM-Net can work on complex schemata with multiple tables (i.e., they can take also relationships and fetaures from other tables into consideration).}

\comments{O7}{While the baseline models cover a wide-spectrum of deep models, there are many relevant alternatives as discussed before (e.g., graph neural networks) and it is not clear why the paper does not compare against those approaches.}

\comments{Response to author feedback C1}{
The arguments to not compare to GNNs are not really convincing. 
Transforming a relational database to a graph to use GNNs is not complicated. I agree that the training efficiency will become a problem for large data sets. However, the accuracy might still be comparable to ARMNet. Hence, I think that a comparison to GNNs is important.}
%%% ooibc: this is reviewer's comment to our earlier response?
% sf: yes, our earlier response is as follows:
% First, we clarify that our main focus is to develop a relation modeling network tailored for structured data, and we formulate structured data as one logical table for ease of discussion. However, we note that ARM-Net can readily work on multiple tables, which can be realized by taking features from relevant tables [15] or adopting the logical table abstraction [11, 29]. Second, GNNs are not ideally suited for relational modeling. GNNs can be described as learning a refined representation for each node, by aggregating and transforming information passed from neighbor nodes [15, a], and then the learned node presentations can be used for prediction. This process can be understood as modeling cross features in an implicit manner, similar to DNNs, which is again ineffective and lacks interpretability. Further, how to model relational data with GNNs is not straightforward. The key to applying GNNs to relational data is how to properly transform structured data into a graph, specifically, clearly defining nodes and their connections. A promising way could be treating each field as a node, and assuming full connection since no prior knowledge about the connection is available, which however leads to time complexity quadratic to the number of fields (linear with ARM-Net). [15] sidesteps this by treating each tuple as a node and the foreign key as a directed connection from one node to another (tuple of another table). This however creates more problems. [15] needs to build a subgraph of nodes and their connections by indexing many other tuples for the prediction of a single target tuple, which is extremely inefficient and may cause a violation of privacy. Briefly, introducing GNNs to structured data is non-trivial, and the only available related work [15] (arxiv) is also problematic. These are the main reasons why we did not adopt GNN methods in experiments. However, we will compare with GNN based approaches as suggested.

\responseArg{O2/O7/C1}{
We have adopted two graph neural network (GNN) baselines as suggested, including the GCN~\cite{gcn} and GAT~\cite{gat} model.
Specifically, we have introduced the two GNN models in Section~\ref{sec:baseline}, included their results in the overall prediction performance summarized in Table~\ref{tab:overall_resutls} and updated the effectiveness discussion in Section~\ref{sec:exp_effectiveness} accordingly.
}

\comments{O3}{Certain contributions of the paper are oversold. For example, the discussion around explainability seems constructed. Sure, one could see the weights as some form of explanation to show the user which cross-attribute features are important for a decision. But this is more a simple by-product of ARM-Net and I do not see this as a separate contribution. Moreover, explaining complex deep models certainly needs much more than showing important cross-attribute features and many approaches exist already. Hence, I would suggest to remove the part centered around explainablity and suggest that the authors use the space to discuss / evaluate potential model alternatives.}

\comments{O10}{The experimental evaluation centered around interpretability could be massively reduced to make space for additional experiments.}

\comments{Response to author feedback C2}{I am still not seeing that interpretability of ARMNet is a major contribution. As also mentioned by Reviewer\#5, this should be toned down since this type of interpretability is quite standard.}

\responseArg{O3/O10/C2}{
We have toned down the interpretability of \name by updating the introduction around interpretability in Abstract and Introduction (the fifth paragraph) and moving the detailed discussion to a separate subsection in Section~\ref{sec:analysis_and_discussion} to clarify how \name is different from existing post-hoc interpretation approaches and how its explicit modeling process may facilitate global/local interpretability in human understandable terms.

We have substantially reduced the experimental evaluation on interpretability in Section~\ref{sec:exp_interpretability} to make space for additional experiments (mostly in Section~\ref{sec:exp_effectiveness} and Section~\ref{sec:exp_ablation}) as suggested.

To make the evaluation of interpretability more objective, we have also introduced two general interpretation approaches, Lime~\cite{lime} and Shap~\cite{shap}, as suggested by Reviewer 3.
The discussions and interpretability results of \name compared against Lime and Shap can be found in Section~\ref{sec:analysis_and_discussion} and Section~\ref{sec:exp_interpretability} respectively.
Specifically, although there exist general post-hoc interpretation approaches explaining how a black box model works, including perturbation based~\cite{lime,shap}, gradient-based~\cite{attributionDNN} and attention-based~\cite{selvaraju2017grad} methods, explanations given by another model is often not reliable, which can be misleading~\cite{xaisurvey,shap}.
Alternatively, \name follows \textit{transparent box design}~\cite{xaisurvey}, which perfectly represents itself with a more transparent modeling process for relational analytics.
The interpretability results in Section~\ref{sec:exp_interpretability} also show that the global feature importance provided by \name is consistent with the two general interpretation approaches, namely Lime and Shap.
However, we note that the interpretation results provided by \name are relatively more reliable since \name inherently supports global feature attribution, and its modeling process is more transparent, whereas Lime and Shap are typically adopted as a medium to interpret other ``black box'' models via approximation.


}

\comments{O4}{The discussion on how an ARM-Net ensemble is learned needs a more careful description.}

\response{
We have updated Section~\ref{sec:optimization} with a more detailed description of how an \name ensemble is learned.
}

\comments{O5}{The choice of which hyper-parameters ARM-Net offers also needs more justification. Why is one size for all hidden layers a good choice? Did you evaluate this in experiments to show that different layer sizes / types would not provide even a better accuracy at the end.}

\response{
In the original manuscript, We did not optimize most hyperparameters and instead simply followed the settings of AFN [13] because they are not key architecture parameters of ARM-Net.

In the revised manuscript, we have updated the implementation of all the baseline models.
Further, for a fair comparison, we evaluate the effectiveness of all the models with the same updated training settings, which is introduced in Section~\ref{sec:hyper_settings}.
The updated results reported in this manuscript are obtained by a thorough grid search of hyperparameters for all the models (over 10k runs in total), each with five independent runs to reduce randomness.
Specifically, the best searched key hyperparameters of \name are provided in Table~\ref{tab:dataset_stats}.
}

\comments{O6}{While the evaluation shows results on a wide spectrum of data sets, the evaluation should make clearer why this is a good selection of data sets. Do they vary in complexity; i.e., degree of correlation between attributes? In addition to real-world data sets, it would be good to see how the model performance compares on synthetic data where individual parameters such as correlation between attributes can be modified on a per tuple-level from highly dependent to independent.}

\response{
We evaluate \name on five real-world relational datasets on representative domains, namely app recommendation (\frappe), movie recommendation (\movielens), click-through rate prediction (\avazu, \criteo) and healthcare (\diabetes)
%%% ooibc: not a subset -- all five
These datasets are widely-adopted benchmarks for the respective domains with different data sizes and numbers of attribute fields.
%%% ooibc: These... these ...
We have clarified the dataset descriptions in Section~\ref{sec:dataset}.
The statistics of these datasets are summarized in Table~\ref{tab:dataset_stats}.

We have compared model performance on synthetic data where the correlation between attributes varies across tuples, and \name achieves consistently better prediction performance than baseline models.
To evaluate the effectiveness of the interaction features dynamically captured by \name, we have also introduced a subsection in Section~\ref{sec:exp_ablation} (\textit{Enhancing FM with Exponential Neurons}).
Specifically, we collect the feature interaction terms in \name and augment the learning of the factorization machine model (FM~\cite{fm}) with these synthetic interaction features.
The results illustrated in Figure~\ref{fig:synthetic} demonstrate that interaction features dynamically captured with the exponential neurons consistently improve the prediction performance of FM by a large margin, even with only a few synthetic interaction features.
}


\comments{O8}{Figure 5/6 are redundant and can be removed.}

\response{
We have removed Figure 5/6 of the original manuscript as suggested.
}

\comments{O9}{The experiments should also compare the training efficiency (in training time) and not only the inference efficiency.}

\response{
We have included the training efficiency in Table~\ref{tab:efficiency} and updated the discussions accordingly in Section~\ref{sec:analysis_and_discussion} and Section~\ref{sec:exp_ablation}.
}

\comments{Required changes for a revision}{Please provide more details as detailed in (O2-O5). Also please provide additional experiments, as requested in (O6,O7,O9).
\newline Moreover, as noted by reviewer\#5, clarify if the numbers for the baseline methods are copied from other papers. And if so, rerun the experiments for the baselines using the same setup as for ARMNet.
\newline Finally, please also provide a reason why no code has been made available.}

\response{
We have provided more details for O2-O5, and provided additional experiments as requested in O6, O7, O9.

We have clarified the numbers for the baseline methods in our response to the meta reviewer and Comment O5 above and rerun the experiments for all the baseline models using the same setup as for \name.
As for the code availability, since a patent is being filed, we only provide the core code~\footnote{\href{https://drive.google.com/file/d/1n9UuBBialylrSzWsVilv5X8Mz8kKBLN-/view?usp=sharing}{https://drive.google.com/armor\_core\_code}} for all the models and corresponding training scripts for reproducibility.
We will open source all the code subsequently upon acceptance.
%%% ooibc: some may view PyTorch negatively

}


\section*{Response to Reviewer 2}


\comments{Original O2}{I think the paper could be greatly improved with a simple example: suppose a table containing monthly sales data has four columns, month, the store ID, the product ID, and the total sales that month. A particular store might perform better at selling a particular product -- interacting (multiplying) a one-hot encoding of the store ID with a one-hot encoding of the product ID, and then performing a logistic regression, would bring this to the forefront quickly. If all stores sell way more of a particular product in December, then "interacting" a one-hot encoding of the month (a "is December" variable) with a one-hot encoding of the product ID would bring this to the forefront. Using a traditional DNN, you'd need many layers to "simulate" the multiplication.}

\response{
We have introduced the suggested example in the Introduction (highlighted in blue in the sixth paragraph of Section~\ref{sec:introduction}), which greatly improves the clarity.
}

\comments{Original O3}{It is difficult for me to tell if this paper presents a new, potentially foundational concept, the "CNN for Database Schemas", or is simply a well-engineered combination of tricks that play well together. Either way, I think this paper meets the threshold for acceptance, but I am frustrated by the lack of clarity.
\\
\\The overall format the authors seem to use for justifying their design choices is "our model weights X could take on value Y, which means our model subsumes alternative model Z, but because of the layout of X, we can do an intepretability analysis." Of course, this is totally technically correct. But I think it is a fundamentally backwards way of thinking about an architecture. This explanation basically makes me think you've found a clever way of modeling previous approaches in a differentiable structure, and the way you've done the modeling is amenable to interpretation.
\\
\\Instead, I'd love to understand how the architecture of ARM-Net biases the model towards learning certain types of features (like how a CNN is biased towards learning local structures that can occur anywhere in an image). If this paper can convey that level of understanding about ARM-Net, it could really be the basis for a wide range of research. As it stands now, I think the work is technically correct, suitably tested, and engages well with prior work. But I'm unable to tell if this is a bag of useful tricks or something fundamental.}

\response{
We have clarified our design choices and rationales behind each module of \name throughout the updated manuscript.
The major updates on the clarification can be found in highlighted paragraphs of Introduction, Section~\ref{sec:overview}, Section~\ref{sec:architecture} and Section~\ref{sec:analysis_and_discussion}.
}

\section*{Response to Reviewer 3}

\comments{O1}{While the focus on interpretability is well appreciated, the 2-page long section 4.3 is largely subjective. Why not compare against an existing interpretable approach such as LIME? That would make the enhanced interpretability of the proposed model at least somewhat objective. Right now, section 4.3 is hard to read, the claims are even harder to digest (I suspect there may be some typos in that section which lead to some confusion).}

\comments{Response to author feedback}{The authors have offered to address O1 by providing a comparison with other post-hoc interpretable approaches. Eager to see that be a part of the paper.}

\comments{Required changes for a revision}{Address O1 by comparing against post-hoc interpretable approach. The authors have offered to provide this in their rebuttal.}

\response{
We have updated the entire interpretability section of Section~\ref{sec:exp_interpretability} and rearranged the interpretation results into three subsections, namely \textit{Interpretability Settings}, \textit{Global Interpretability} and \textit{Local Interpretability}.

In particular, we have provided a detailed introduction of the interpretability settings and compared both global and local interpretability results of \name against two post-hoc interpretable approaches as suggested, including Lime~\cite{lime} and Shap~\cite{shap}, which are two widely-adopted input perturbation interpretation methods based on linear regression
and game theory respectively to identify the feature importance of the models to be interpreted.
These updates indeed make the enhanced interpretability of \name more objective.
Detailed discussions and interpretability results can be found in the newly introduced subsection in Section~\ref{sec:analysis_and_discussion} and Section~\ref{sec:exp_interpretability}.
}

\comments{Additional remarks}{I'll use this portion of the review to make some suggestions. In section 4.3.1, I come across statements such as "Neuron1 ... assigns more interaction weights to {user\_id, item\_id, is\_free}...". Similarly, "Neuron3" is said to identify "user\_id, weather". Interpretability is only useful if the model informs us about the data/domain being modeled. I am assuming the authors, with their statements, are implying that the cross-correlations ARM-Net identifies are indeed correlations that hold for the Frappe data. I see nothing in section 4.3 to imply that these cross-correlations are indeed cross-correlations that hold for the Frappe data and are not, for instance, spurious correlations. That's the main issue I have with section 4.3. The reader needs some confirmation that these correlations are not aberrations introduced by ARM-Net. This is just a suggestion but we could for instance, apply a post-hoc interpretability technique such as LIME and if LIME also uncovers these purported correlations then I'd be more inclined to believe that these are indeed genuine correlations. A lot of NLP papers (especially ones positing that attention can be used to aid interpretability) display anecdotal evidence by showing the sentence and highlighting the words that led to the prediction. Perhaps you can show some records/tuples where the purported correlations are 'highlighted' to show how these aid prediction. If the authors don't want to take my suggestions and can find a different way to justify the correlations they claim ARM-Net found then I'd be fine with that too. Currently, section 4.3 seems to be light on any kind of justification for the correlations found by ARM-Net. I think that sort of justification is necessary and without it section 4.3 is of questionable value. Evaluation in XAI is notoriously hard but that does not mean we stop evaluating or refrain from comparing with other interpretability techniques. I hope this feedback is of some use to the authors and helps them improve upon the paper.
\\
\\Another suggestion would be to check recent surveys on XAI to relate your approach in terms of XAI taxonomies that have recently been compiled. See for instance, 2018 ACM Survey by Guidotti et al.
\\
\\Last line on page 10 (which continues onto page 11) mentions both Neuron3 and Neuron1. Which one do you mean?}

\response{
We have taken the suggestion by highlighting the importance of input features provided by \name and comparing these results with other post-hoc interpretation approaches (Lime~\cite{lime} and Shap~\cite{shap}) in Figure~\ref{fig:global_frappe_diabetes}, Figure~\ref{fig:local_frappe}, Figure~\ref{fig:lime_shap_frappe}, Figure~\ref{fig:local_diabetes} and Figure~\ref{fig:lime_shap_diabetes}.
Further, we have included the global interaction terms captured by \name in Table~\ref{tab:frappe_interaction_terms} and Table~\ref{tab:diabetes_interaction_terms} to show the most frequently captured feature correlations.

The discussions and interpretability results of \name compared against Lime and Shap can be found in Section~\ref{sec:analysis_and_discussion} and Section~\ref{sec:exp_interpretability} respectively.
Specifically, although there exist general post-hoc interpretation approaches explaining how a black box model works, including perturbation based~\cite{lime,shap}, gradient-based~\cite{attributionDNN} and attention-based~\cite{selvaraju2017grad} methods, explanations given by another model is often not reliable, which can be misleading~\cite{xaisurvey,shap}.
Alternatively, \name follows \textit{transparent box design}~\cite{xaisurvey}, which perfectly represents itself with a more transparent modeling process for relational analytics.
The interpretability results in Section~\ref{sec:exp_interpretability} also show that the global feature importance provided by \name is consistent with the two general interpretation approaches, namely Lime and Shap.
However, we note that the interpretation results provided by \name are relatively more reliable since \name inherently supports global feature attribution, and its modeling process is more transparent, whereas Lime and Shap are typically adopted as a medium to interpret other ``black box'' models via approximation.

We have also introduced a subsection in Section~\ref{sec:exp_ablation} (\textit{Enhancing FM with Exponential Neurons}) to show the effectiveness of the interaction features captured by \name.
Specifically, we collect the feature interaction terms in \name and augment the learning of the factorization machine model (FM~\cite{fm}) with these interaction features.
The results illustrated in Figure~\ref{fig:synthetic} demonstrate that interaction features dynamically captured with the exponential neurons consistently improve the prediction performance of FM by a large margin, even with only a few captured interaction features.

We have related our approach in terms of XAI taxonomies in the newly introduced \textit{Interpretability} subsection in Section~\ref{sec:analysis_and_discussion} and corrected the typo in the interpretability description.
}


\section*{Response to Reviewer 5}

\comments{W1}{Newer architectures such as graph neural network are omitted from the comparison. Especially, since novelty is claimed for these structured datasets this omission is not appropriate.}

\response{
We have adopted two graph neural network (GNN) baselines as suggested, namely the GCN~\cite{gcn} and GAT~\cite{gat} model.
Specifically, we have introduced the two GNN models in Section~\ref{sec:baseline}, included their results in the overall prediction performance summarized in Table~\ref{tab:overall_resutls} and updated the effectiveness discussions in Section~\ref{sec:exp_effectiveness} accordingly.
}

\comments{W2}{Interepretability is one contribution of this paper. However, interpretability through attention is quite standard. Overall, model interpretability techniques may not work well and in fact may be confusing (https://arxiv.org/abs/1802.07810, https://arxiv.org/abs/1606.03490).
The motivating case stated for interpretability is healthcare. However, clinical data is usually time-series data and the techniques presented here won't apply easily or will likely lead to sub-optimal results.
This is not a problem with just this paper. But showing some feature importance scores does not mean that they are useful for the task at hand.}

\comments{Required changes for a revision}{Please tone down the interpretability motivation and claims. and also include critical results in the discussion.
You need to address W2 and W3 which is only about writing and overselling your results. I think the experimental results speak for themselves.
While for interpretability the experimental results do not tell us much. So say that your method's ability to determine the importance of feature interactions rather than single feature values may lead to improved interpretability.
The claims about interpretability do not hold up to what is delivered . You need to revise the text to say that the new architecture captures feature interactions as first class objects that may improve interpretability compared to standard DNN with existing interpretability methods. Please note the "may" as you have not demonstrated this to be the case.}

\response{
We have toned down the interpretability of \name by updating the introduction of interpretability in Abstract and Introduction (the fifth paragraph) and moving the detailed discussion to a separate subsection in Section~\ref{sec:analysis_and_discussion} to clarify how \name is different from existing post-hoc interpretation approaches and how its explicit modeling process may facilitate global/local interpretability in human understandable terms.

We have updated our discussions accordingly and substantially reduced the experimental evaluation of interpretability in Section~\ref{sec:exp_interpretability} to make space for additional experiments (mostly in Section~\ref{sec:exp_effectiveness} and Section~\ref{sec:exp_ablation}) instead.

To make the evaluation of interpretability more objective, we have also introduced two general interpretation approaches Lime~\cite{lime} and Shap~\cite{shap} as suggested by Reviewer 3.
The discussion and interpretability results of \name compared against Lime and Shap can be found in Section~\ref{sec:analysis_and_discussion} and Section~\ref{sec:exp_interpretability} respectively.
Specifically, although there exist general post-hoc interpretation approaches explaining how a black box model works, including perturbation based~\cite{lime,shap}, gradient-based~\cite{attributionDNN} and attention-based~\cite{selvaraju2017grad} methods, explanations given by another model are often not reliable, which can be misleading~\cite{xaisurvey,shap}.
Alternatively, \name follows \textit{transparent box design}~\cite{xaisurvey}, which perfectly represents itself with a more transparent modeling process for relational analytics.
The interpretability results in Section~\ref{sec:exp_interpretability} also show that the global feature importance provided by \name is consistent with the two general interpretation approaches, namely Lime and Shap.
% kp: "feature importance" v.s. "feature attribution" are used interchangeably throughout the paper - better be consistent
% feature attribution -> an interpretation approach, mostly refer to producing feature importance for input features
However, the interpretation results provided by \name should be relatively more reliable since \name inherently supports global feature attribution, and its modeling process is more transparent, whereas Lime and Shap are typically adopted as a medium to interpret other ``black box'' models via approximation.
% kp: why "since \name inherently supports global feature attribution"? i think how to generate global feature attribution is similar for ARM-Net and LIME, SHAP?
% lime/shap -> interpretation approaches that interpret other models
% armnet -> inherently support interpretation
}

\comments{W3}{The spin about structured data is not really convincing - these are standard datasets and have been experimented on exhaustively. Claiming that DNNs work well for speech, text, images but not structured data, is simply not right.
In fact, I find that SIGMOD may not be the right conference for this paper. However, I think the audience may find this interesting as they start to branch more into ML territory.}

\response{
We have updated the discussion in the Introduction (mainly in the second paragraph) accordingly to clarify why DNNs may not be ideal for structured data.
The main justifications are as follows.
There are intrinsic correlations and dependencies among attribute values of structured data, and such feature interactions are essential for predictive analytics.
Although theoretically a DNN can approximate any target function given sufficient data and capacity, the interactions captured for a conventional DNN layer are additive.
As a result, prohibitively large and increasingly inscrutable models that stack multiple layers with nonlinear activation functions in-between are required to model such multiplicative interactions~\cite{multiplicative,latentcross}.
Previous studies~\cite{afn,latentcross,polynomialnn,multiplicative} have also suggested that modeling such ``cross features'' implicitly with DNNs may take a substantial number of hidden units, which greatly increases the computational cost and at the same time renders it difficult to be interpreted.
% kp: "it" -> "the DNNs"?
% it -> modeling such ``cross features'' implicitly with DNNs

We have also introduced three neural network based models as baselines to support this contention, including DNN, GCN~\cite{gcn} and GAT~\cite{gat} in Section~\ref{sec:experiment}.
The results of these NN-based models are included in Table~\ref{tab:overall_resutls} and discussed in Section~\ref{sec:exp_effectiveness} (\textit{NN-based Models and Ensemble Models}).
We summarize the main findings as follows.
(1) Despite not explicitly modeling feature interactions, the best NN-based models generally achieve strong prediction performance against other single model baselines.
Particularly, the attention-based graph network GAT obtains noticeably higher AUC than other single models on \avazu and \diabetes.
However, their performance varies greatly across different datasets, which is not as consistent as \name.
(2) Model ensembles with a DNN significantly improve their respective predictive performance.
This can be observed consistently throughout the baseline models, e.g., DCN+, xDeepFM and AFN+, which suggests that the nonlinear interactions captured by DNNs are complementary to explicitly captured interactions.
(3) \name achieves comparable performance with DNN, and \nameplus further improves the performance considerably, which obtains the overall best performance across all the benchmark datasets.
These results further confirm the effectiveness of \name in modeling feature interactions of arbitrary orders in a selective and dynamic manner.
}


\end{multicols}
